Causal Discovery in the Presence of Missing Data

Missing data are ubiquitous in many domains including healthcare. When these data entries are not missing completely at random, the (conditional) independence relations in the observed data may be different from those in the complete data generated by the underlying causal process. Consequently, simply applying existing causal discovery methods to the observed data may lead to wrong conclusions. In this paper, we aim at developing a causal discovery method to recover the underlying causal structure from observed data that follow different missingness mechanisms, including missing completely at random (MCAR), missing at random (MAR), and missing not at random (MNAR). With missingness mechanisms represented by missingness graphs, we analyse conditions under which additional correction is needed to derive conditional independence/dependence relations in the complete data. Based on our analysis, we propose the Missing Value PC (MVPC) algorithm for both continuous and binary variables, which extends the PC algorithm to incorporate additional corrections. Our proposed MVPC is shown in theory to give asymptotically correct results even on data that are MAR or MNAR. Experimental results on synthetic data show that the proposed algorithm is able to find correct causal relations even in the general case of MNAR. Moreover, we create a neuropathic pain diagnostic simulator for evaluating causal discovery methods. Evaluated on such simulated neuropathic pain diagnosis records and the other two real world applications, MVPC outperforms the other benchmark methods.

==> simulator.tex <==
\section{Neuropathic pain diagnosis simulator for the evaluation of causal discovery algorithms} \label{sec:simulator}
The evaluation of causal discovery methods is lack of real-world benchmark datasets, which has been a challenge \citep{pannel2018}. Ground-truth causal relations of a complex real-world scenario are often unknown, thus synthetic data sampled from randomly generated causal graphs are commonly used for the evaluation. However, such synthetic data are mostly based on the model proposed in a work such that it could be hard to be used for the evaluation of \hk{the works of} others. Moreover, the synthetic data experiments may show the superior performance of proposed methods but sometimes may oversimplify the challenges in real-world scenarios \citep{garant2016evaluating}. Fortunately, towards tackling the evaluation challenge, domain experts in  disciplines such as biology and physics can provide well-understood causal influences in some specific scenarios. This can give us opportunities to utilize domain knowledge to reveal ground-truth causal relations and build realistic simulators. In this way, we can generate data from simulators and use them as benchmark datasets for the evaluation of causal discovery algorithms.
 
In this section, we introduce our neuropathic pain diagnosis simulator that can be used for the evaluation of causal discovery algorithms.\footnote{ The simulator is available at \href{https://github.com/TURuibo/Neuropathic-Pain-Diagnosis-Simulator}{https://github.com/TURuibo/Neuropathic-Pain-Diagnosis-Simulator}.} 
We first show essential causal relations in the neuropathic pain diagnosis, and then present details of the simulator design. 
\rt{Other details, e.g., simulating the data in the presence of unknown confounding, selection bias, or missing data, can be found in \citep{tu2019neuropathic}.}

\begin{table}[htb]%\[!htb\]
    \caption{Diagnostic records and dataset.} % all dataset, no data set in thi paper
    \begin{subtable}[t]{\textwidth}
        \caption{A typical neuropathic pain diagnostic record. "L" and "R" stand for "left" and "right".} 
        \label{tab:real-rec}
        \center 
            \begin{tabular}{|l|}
            % \center
                \hline
                \textbf{Symptom diagnosis:} 
                R back thigh discomfort, R knee discomfort, \\
                L knee thigh discomfort, Patellofemoral pain syndrome \\ \hline
                \textbf{Pattern diagnosis:} 
                L L5 Radiculopathy, R L5 Radiculopathy                                                            \\ \hline
                \textbf{Pathophysiological diagnosis:} 
                Discoligment injury L4-5                                                               \\ \hline
            \end{tabular}
    \end{subtable}%
    
   \begin{subtable}[t]{\textwidth} \vspace{3mm}
        \center
        \caption{Given many patient records, a diagnostic record dataset takes the following form. "ID" represents different patients. "DLI" and "Radi" stand for discoligamentous injury and radiculopathy. Each row is a patient's diagnostic record in which "1" represents that the patient has the symptom and "0" represents that the patient has no such symptom.}\label{tab:sim-rec}
       \begin{tabular}{ccccccccc}
        \hline
        ID  & DLI C1-C2 & DLI C2-C3 & ... & L C5 Radi & ... & R knee & L neck & ... \\ \hline
        1   & 0         & 0         & ... & 1         & ... & 1      & 0      & ... \\
        2   & 1         & 0         & ... & 0         & ... & 0      & 1      & ... \\
        ... & ...       & ...       & ... & ...       & ... & ...    & ...    & ... \\
        n   & 0         & 1         & ... & 0         & ... & 0      & 0      & ... \\ \hline
        \end{tabular}
    \end{subtable}
\end{table}

\subsection{Causal relations for neuropathic pain diagnosis} \label{sec:gt_cg}
Neuropathic pain diagnoses mainly contain symptom diagnosis, pattern diagnosis, and pathophysiological diagnosis. For example, Table \ref{tab:real-rec} shows typical neuropathic pain diagnostic records. 
\emph{Symptom diagnosis} describes the discomfort of patients. 
\emph{Pattern diagnosis} identifies symptom patterns. In neuropathic pain diagnosis, it identifies which set of nerves do not work properly. Such conditional is commonly called Radiculopathy. The main tool of pattern diagnosis is the dermatome map as shown in Figure \ref{fig:dermatone_map}. 
\emph{Pathophysiological diagnosis} refers to the original cause of symptoms where discoligamentous injury is the most common factor in the neuropathic pathophysiological diagnosis. Given a set of patient data, we can present the data as in Table \ref{tab:sim-rec}, where $1$ indicates that the diagnostic label exists in a patient record and $0$ otherwise.

\begin{figure}
\begin{minipage}[c]{0.4\textwidth}
\centering
\vspace{-9mm}
\includegraphics[width=\textwidth]{figures/Dermatone_map.png}
\captionof{figure}{Dermatome map (image source \cite{dermatone}) shows surface regions of different nerves.}
\label{fig:dermatone_map}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\textwidth}
\centering
\input{tikz/ground_true_graph.tex}
\captionof{figure}{Typical structure of the ground-truth causal graph. "DLI" and "Radi" represent discoligamentous injury and radiculopathy. "shldr" and "im" stand for shoulder and impingement. "L" and "R" stand for left and right. We show the left side symptoms, and the corresponding connections are the same on the right side. 
}
\label{fig:subtree}
\end{minipage}
\end{figure}

In neuropathic pain diagnoses causal relations are well studied in biomedical research \citep{ohnmeiss1999relation,tanaka2006cervical}. In general, neuropathic pain symptoms in symptom diagnosis are mainly caused by radiculopathies (Radi) in the pattern diagnosis, and the radiculopathy is mostly caused by discoligamentous injuries (DLI) in the pathophysiological diagnosis. For example, some of the causal relations are shown in Figure \ref{fig:subtree}. DLI C4-C5 causes left side C5 radiculopathy and right side C5 radiculopathy. Left side C5 radiculopathy further causes symptoms at the left front shoulder, the left lateral arm, etc. We see that these locations are consistent with the dermatome map in Figure \ref{fig:dermatone_map}. Despite that there are other causes of neuropathic pain symptoms and radiculopathies such as tumors and diabetes, they rarely appear in primary care. Therefore, we focus on the  causal relations among the discoligamentous injuries, radiculopathies, and neuropathic pain symptoms in this work. 

The complete causal relations are summarized in \rt{\citep{tu2019neuropathic}}, and we further provide interactive causal graph visualization at: \url{https://cutt.ly/BekNFSy}. The causal graph is similar to Figure \ref{fig:subtree} and  consists of three layers: Symptom diagnosis, pattern diagnosis, and pathophysiological diagnosis. Nodes in each layer have no connection with each other. Arrows either point from nodes in the pathophysiological diagnosis layer to nodes in the pattern diagnosis layer or from nodes in the pattern diagnosis layer to nodes in the symptom diagnosis layer. The causal graph also contains different d-separations such as the folk structure, denoted by $\wedge$ structure (e.g., Left C$5$ Radiculopathy  $\leftarrow$ Discoligamentous injury C$4$-C$5$ $\rightarrow$ Right C$5$ Radiculopathy), the collider structure, denoted by $\vee$ structure (e.g., Left C$5$ Radiculopathy $\rightarrow$ Left neck pain $\leftarrow$ Left C$4$ Radiculopathy), and the chain structure (e.g., Discoligamentous injury C$4$-C$5$ $\rightarrow$ Left C$5$ Radiculopathy $\rightarrow$ Left Neck pain). 

\subsection{Neuropathic pain diagnosis simulator} \label{sec:npsim}
With the domain knowledge mentioned in Section \ref{sec:gt_cg}, we create our simulator to generate patient diagnostic records. 

\paragraph{Real-world diagnostic records.}
To make our generated records close to the real-world scenario, we learn parameters from a dataset including 141 patient diagnostic records \citep{zhang2016diagnostic}. \footnote{ The dataset is collected in a hospital department specialized in neuropathic pain \citep{zhang2016diagnostic}. Only Ruibo Tu and Bo C.~Bertilson get access to the dataset during the course of the project.} These patients' diagnostic records are represented as a table of binary variables as shown in Table \ref{tab:sim-rec}. The variables in the pathophysiological diagnosis consist of the craniocervical junction injury and $26$ discoligamentous injuries; the variables in the pattern diagnosis include $52$ radiculopathies; the variables in the symptom diagnosis contain $143$ symptoms. Similar to the real-world diagnostic records, the columns of generated records are the mentioned variables and the rows represent the synthetic patients.

\paragraph{Parameter estimation of the causal graph.} We estimate the Conditional Probability Distribution (CPD) of each variable given its parents in the causal graph with the real dataset. We compute the CPD of a variable $X$ by $P(X \mid Pa(X)) = \frac{P(X, Pa(X))}{P(Pa(X))}$, where $Pa(X)$ represents the parents of $X$ in the causal graph. Since variables are binary, the joint distributions  can be computed using the number of variable values in the dataset. However, we cannot estimate the CPDs accurately for the variables with many parents because of the curse of dimensionality and the limited number of the real data. Therefore, instead of computing the CPD of $X$ given all its parents, we introduce the heuristic 

\begin{equation}\label{eq:app}
P(X=1 \mid Pa(X)=\mathbf{c}) \gets \max_{i\,\in\, I_1} P(X=1\mid Pa_i(X)=c_i),
\end{equation}

where $\mathbf{c}$ is a given vector of parent values (which can contain either value zero or one), and $I_1$ is a subset of the index of all variables in $Pa(X)$ such that for $\forall \, i \in I_1$, $Pa_i(X)\in Pa(X)$ and $c_i=1$. The condition of Equation \ref{eq:app} is that there exists $c_i \in \mathbf{c}$ such that $c_i = 1$. This condition is satisfied in the real data. Given the parent values $\mathbf{c}$, we only consider the parents taking the value one, and get the maximum conditional probability of $X=1$ given a parent taking the value one in $\mathbf{c}$ to estimate the CPD of $P(X=1 \mid Pa(X) = \mathbf{c})$. 

This approximation is supported by the medical insights. Intuitively, if a symptom is caused by multiple nerves, the chance for the symptom to exist in general is higher when these causes occur at the same time comparing to only one of the causes occurs. For example, both $L4$ and $L5$ radiculopathies can cause knee pain. The chance that a person with both $L4$ and $L5$ radiculopathies feels knee pain is higher or equal to the chance that a person with either one of the radiculopathies feels knee pain. In other words, $P(X=1 \mid Pa_1(X)=1, Pa_2(X)=1) \ge P(X=1 \mid Pa_1(X)=1)$ and $P(X=1 \mid Pa_1(X)=1, Pa_2(X)=1) \ge P(X=1 \mid Pa_2(X)=1)$, where $Pa_1(X)$ and $Pa_2(X)$ are $L4$ and $L5$ radiculopathies and $X$ is knee pain. 

Given all the conditional probability and marginal probability distributions, we use ancestral sampling to sample neuropathic pain diagnosis data of synthetic patients. 
